Computer-Aided Layout Generation for Building Design: A Review

Generating realistic building layouts for automatic building design has been studied in both the computer vision and architecture domains. Traditional approaches from the architecture domain, which are based on optimization techniques or heuristic design guidelines, can synthesize desirable layouts, but usually require post-processing and involve human interaction in the design pipeline, making them costly and timeconsuming. The advent of deep generative models has significantly improved the fidelity and diversity of the generated architecture layouts, reducing the workload by designers and making the process much more efficient. In this paper, we conduct a comprehensive review of three major research topics of architecture layout design and generation: floorplan layout generation, scene layout synthesis, and generation of some other formats of building layouts. For each topic, we present an overview of the leading paradigms, categorized either by research domains (architecture or machine learning) or by user input conditions or constraints. We then introduce the commonly-adopted benchmark datasets that are used to verify the effectiveness of the methods, as well as the corresponding evaluation metrics. Finally, we identify the well-solved problems and limitations of existing approaches, then propose new perspectives as promising directions for future research in this important research area. A project associated with this survey to maintain the resources is available at awesome-building-layout-generation.

==> figs/teaser.tex <==
\begin{figure*}[!htb]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{ccc}

    \centering
        {\includegraphics[width=0.28\linewidth]{figs/teaser/1-1_floorplan.jpg}} &  
        {\includegraphics[width=0.28\linewidth]{figs/teaser/1-2_scene.jpg}} &  
        {\includegraphics[width=0.28\linewidth]{figs/teaser/1-3_other.jpg}}\\


        Floorplan Layouts & Scene Furniture Layouts & Other Types of Building Layouts \\

    \end{tabular}
    \caption{The diverse building layout types used in mainstream computer-aided architectural design methods. The floorplan and scene furniture layouts are the two most common types of layouts. Moreover, there exist other types including roofs, building volumes, community or urban-level layout, etc. The sampled floorplan layouts are referred and rendered from RPLAN~\cite{wu2019data} datasets. The sampled scene furniture layouts are referred from ATISS~\cite{paschalidou2021atiss}. The sampled other building layouts are referred from the following works:~\cite{qian2021roof, chang2021building, fan2023automated, he2023globalmapper}.}
    \label{fig::teaser}
\end{figure*}
